Rethinking Data Shapley for Data Selection Tasks: Misleads and Merits

Data Shapley provides a principled approach to data valuation and plays a crucial role in data-centric machine learning (ML) research. Data selection is considered a standard application of Data Shapley. However, its data selection performance has shown to be inconsistent across settings in the literature. This study aims to deepen our understanding of this phenomenon. We introduce a hypothesis testing framework and show that Data Shapley's performance can be no better than random selection without specific constraints on utility functions. We identify a class of utility functions, monotonically transformed modular functions, within which Data Shapley optimally selects data. Based on this insight, we propose a heuristic for predicting Data Shapley's effectiveness in data selection tasks. Our experiments corroborate these findings, adding new insights into when Data Shapley may or may not succeed.

==> ROC.tex <==
\textbf{ROC Curve for Shapley value-based Hypothesis Testing.} 
Receiver operating characteristic (ROC) curve is a standard tool for assessing the performance of a hypothesis test. The curve is plotted with True Positive Rate on the $y$-axis and False Positive Rate (i.e., 1- True Negative Rate) on the $x$-axis. Each point on the ROC curve represents a TP/FP pair corresponding to a particular decision threshold being used in a hypothesis test. The diagonal line that runs from the bottom left (0, 0) to the top right (1, 1) represents a scenario where $\Spec(\testfunc) + \Sens(\testfunc) = 1$, which represents the baseline of random guessing. The higher the ROC curve is, the better the hypothesis test is. 

We evaluate the ROC curve for comparing the utility of two different data subsets $\U(S_1)$ and $\U(S_2)$. 
To conduct the hypothesis test, we use the natural hypothesis test of comparing the sum of the Shapley values for data points in a subset $S$, i.e., 
$\testfunc(\phi) = 
\ind\left[ \phi[S_1]-\phi[S_2] \ge \alpha \right]$. 
The threshold $\alpha \in \R$ is varied to obtain the ROC curve. We uniformly sample pairs of data subsets of the same sizes and apply the Shapley value-based hypothesis test to predict which data subset possesses greater utility. 
The results are shown in Figure \ref{fig:ROC-main}. For each dataset, we create its noisy variants by randomly picking a certain proportion of the data points to flip their labels. Since mislabeled data usually negatively affect the model performance, its marginal contribution will likely be worse than any other clean data points, mirroring the utility function structure described in Theorem \ref{thm:structureV}. 
As we can see, for clean datasets, the ROC curve is close to a random guess. However, as the proportion of mislabeled data points increases, the effectiveness of the Shapley value-based hypothesis test improves. This observation is consistent with the discussion in Sections \ref{sec:when-fail} and \ref{sec:when-success}, reinforcing the notion that Data Shapley's effectiveness is enhanced in scenarios where the utility functions follow specific structural patterns.

% This aligns with the discussions in Section \ref{sec:when-fail} and \ref{sec:when-success} that Data Shapley is more effective when the underlying utility functions exhibit certain structures. 

\begin{figure*}[h]
    \centering
    \setlength\intextsep{0pt}
    \setlength\abovecaptionskip{0pt}
    \setlength\belowcaptionskip{0pt}
    \includegraphics[width=\linewidth]{images/ROC-main_2.pdf}
    \caption{ROC curves for comparing dataset utilities with Shapley value-based hypothesis test. We show the results when each pair of $S_1, S_2$ is uniformly sampled from the full dataset of size equal to $0.3n$, $0.5n$, and $0.7n$.} 
    \label{fig:ROC-main}
\end{figure*}



==> broader-impact.tex <==
\section*{Broader Impact}
This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here. 



==> failure_exp.tex <==

\subsection{Exploring Shapley Failures in Practical Scenarios}

In this section, we provide empirical results augmenting Theorem \ref{thm:hypo-random} .  

% \tianhao{we call $\U$ utility functions} [checked]
In Theorem \ref{thm:hypo-random} , we show that for \textit{free} utility functions $v: 2^{S} \to \mathbb{R}$ , decision algorithm $h$ only utilizing Shapley value $\phi(\cdot\,;v): S\to \mathbb{R}$ performs no better than random guess in deciding whether $v(S_1) > v(S_2)$ for $S_1,S_2\subset S$. However, in practical scenarios, we usually deal with \textit{constrained} utility functions, which may dismiss the 
impossibility results of Theorem \ref{thm:hypo-random} . In this section, we explore the cases of constrained utility functions and empirically show Shapley values do give misleading results in practice. As we expect a datum with larger Shapley value to be more favorable, we additionally suppose there exists function $g: \bigcup_{S'\subset S}(S' \to \mathbb{R}) \to \mathbb{R}$ that monotonically increases with each input dimension and $h(\phi(S_1\,;v), \phi(S_2\,;v))$ monotonically increases with $g(\phi(S_1\,;v)) - g(\phi(S_2\,;v))$ if we view elements of type $(S'\to \mathbb{R})$ as variable-length vectors. 

\textbf{Experiment Setup. } In this experiment, utility functions are classification accuracy on different validation sets. We use $v_{({\cal V}, {\cal A})}$ to represent the utility function determined by validation set ${\cal V}$ and classifier training algorithm ${\cal A}$. We set ${\cal A}$ to be a $5$-nearest neighbor classifier. 
% , while our proposed method extends to other classifier training algorithms. 
For different training data selection size $k$, we find $S_1$ of size $k$ such that it maximizes $g(\phi(S_1\,; v_1))$, and $S_2$ to be a randomly selected dataset of size $k$. By selecting different validation sets ${\cal V}_1$ and ${\cal V}_2$, we try to find a pair of utility functions $v_1 = v_{({\cal V}_1, {\cal A})}$ and $v_2 = v_{({\cal V}_2, {\cal A})}$ results in the same data selection decision for $h$ satisfying the condition, while one and only one of the arguments $v_1(S_1) < v_1(S_2)$, $v_2(S_1) < v_2(S_2)$ holds, as the case illustrated in Figure \ref{fig:illustration-proof} . To find instances of $v_1$ and $v_2$, we propose Algorithm \ref{alg:worst-case-exploration} . For each chosen $k$, we set $v_1$ the full validation set and utilize Algorithm \ref{alg:worst-case-exploration} to find a $v_2$, Figure \ref{fig:worst-case-exploration} plot $v_1(S_1)$, $v_2(S_1)$, $v_1(S_2)$ and $v_2(S_2)$ for each chosen $k$ . Selection capacities $k$ present as selection percentages in Figure \ref{fig:worst-case-exploration} . 

We can see that $(v_1(S_1) - v_1(S_2))(v_2(S_1) - v_2(S_2)) \le 0$ while $S_1$ is the best subset according to Shapley values $\phi(\cdot\,;v_1)$ and $\phi(\cdot\,;v_2)$, testifying our theoretical results. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{images/experiment-1-all.png}
    \caption{Experiments on OpenML Datasets}
    \label{fig:worst-case-exploration}
\end{figure}

\clearpage

\begin{algorithm}[h]
   \caption{Worst Case Exploration}
   \label{alg:worst-case-exploration}
\begin{algorithmic}
    % Try to make it "flat"
    \INPUT training set selection size $k$ 
    \INPUT dataset $S_1$ selected using Shapley values
    \INPUT dataset $S_2$ selected randomly
    \INPUT training set $S_{\cal T}=\{(x_i, y_i): i\in [1 \dots I]\}$
    \INPUT validation set $S_{\cal V}=\{(\hat x_j, \hat y_j): j\in [1 \dots J]\}$
    \INPUT classifier training algorithm ${\cal A}$
    \STATE suppose $S_{\cal T}$ is sorted such that $\phi(i; v_{(S_{\cal V}, {\cal A})}) < \phi(i+1; v_{(S_{\cal V}, {\cal A})})$
    \STATE declare linear programming problem $LP := \{\}$ . 
    \STATE declare boolean variables $\{z_j: j\in [1 \dots J]\}$ in $LP$
    \STATE train a classifier $M$ on $S_1$ using ${\cal A}$
    \STATE declare boolean $\hat z_j$ indicating $M$ predicts $(\hat x_j, \hat y_j)$ correctly 
    \STATE train a classifier $M'$ on $S_2$ using ${\cal A}$
    \STATE declare boolean $\hat z_j'$ indicating $M'$ predicts $(\hat x_j, \hat y_j)$ correctly 
    \STATE compute $\phi_{ij} = \phi(i; v_{(\{(\hat x_j, \hat y_j)\}, {\cal A})})$
    \STATE declare boundary variable $b$ in linear programming problem $LP$ . 
    \STATE for $i < k$ add constraints $\phi_{ij}\cdot z_j \le b$ to $LP$ . 
    \STATE for $i \ge k$ add constraints $\phi_{ij}\cdot z_j \ge b$ to $LP$ . 
    \IF{$v_{(S_{\cal V}, {\cal A})}(S_1) < v_{(S_{\cal V}, {\cal A})}(S_2)$}
        \STATE solve LP maximizing $(\hat z_j - \hat z_j')\cdot z_j$
    \ELSE
        \STATE solve LP minimizing $(\hat z_j - \hat z_j')\cdot z_j$
    \ENDIF
    \STATE {\bf return} $S_{\cal V}' := \{(\hat x_j, \hat y_j) : z_j = 1\}$ {\quad\tt // selected validation dataset}
\end{algorithmic}
\end{algorithm}

The above algorithm utilized mixed integer programming to select parts of the validation set. First, we compute Shapley values from the training set and the full validation set, and select a subset $S_1$ of the highest $k$ Shapley values. Then, for each instance $j$ in validation set, we compute Shapley values $\phi_{ij}$ for each training set element $i$ . Then, we use a list of Boolean variables $z_j$ to represent the selection of validation set, the Shapley values can be computed as $\phi_{i} = \sum_{j}z_j\phi_{ij}$ . When $S_1$ , the Shapley selected set outperforms $S_2$, the random selected set, we try to find $z_j$ such that $S_1$ is still the Shapley selected set suggesting the hypothesis testing gives the same result while on the selected validation set $S_{\cal V}' := \{(\hat x_j, \hat y_j) : z_j = 1\}$ the model trained on $S_2$ outperforms the modeled trained on $S_1$ . Similarly, we can also solve $z_j$ for cases where $S_2$ outperforms $S_1$. 

\clearpage

==> justification-for-heuristic.tex <==


\section{Justification for Heuristic
\tianhao{remove}
}
\label{appendix:justification-heuristic}

In Appendix \ref{appendix:justification-heuristic}, we provide a theoretical guarantee of such a heuristic under the condition that the fitted $\Ualter$ is within the ``safety-margin'' of $\U$ (a measure for data values' rank stability defined in \citet{wang2023data}). Specifically, we show that the fitting residual is an upper bound for the discrepancy between the utility of the subset selected by Data Shapley, $\ShapleySet^{(k)}$, and the optimal subset, $\optS^{(k)}$. While the safety-margin is hard to compute in practice, it justifies the effectiveness of such a heuristic. 

\begin{definition}[Safety Margin for a specific utility function $\U$]
\label{def:safetymargin}
We denote the difference between the Shapley value of two data points $i$ and $j$ as $D_{i, j}(\U) := \phi_{i}(\U) - \phi_{j}(\U)$. We define the safety margin of a utility function $\U$ as the maximum amount of noise such that for any $\widehat \U$ where $\norm{\widehat \U - \U} \le \safe(\U)$, we have 
$$
D_{z_i, z_j}(\U) D_{z_i, z_j}(\widehat \U) \ge 0
$$
for any pair of $z_i, z_j \in D$. 
\end{definition}
If we know $\U$, we can compute $\safe(\U)$ via the method shown in the proof of Lemma C.1 in \cite{wang2023data}. 

\begin{theorem}
    For any utility function $\U$, if there exists a $\Ualter$ s.t. $\Ualter$ can be written as $\Ualter(S) = f(\sum_{z_i \in S} w_{z_i})$ for some monotonic $f$ and weights $\{w_{z_i}\}_{i=1}^{N}$, and $\norm{\Ualter - \U} \le \safe(\U)$, then let 
    \begin{align}
        \phiS &= 
        \argmax_{S: |S|=k} \sum_{z_i \in S} \phi_{z_i}(\U) \\
        \optS^{(k)} &= \argmax_{S: |S|=k} \U(S)
    \end{align}
    Then we have 
    \begin{align*}
        \U( \phiS ) \ge \U( \optS^{(k)} ) - 2 \norm{\Ualter - \U}
    \end{align*}
\end{theorem}
\begin{proof}
Obviously, we have 
    \begin{align}
        &\left| \U(\phiS) - \Ualter(\phiS) \right| \le \norm{\Ualter - \U} \label{eq:one} \\
        &\left| \U(\optS^{(k)}) - \Ualter(\optS^{(k)}) \right| \le \norm{\Ualter - \U}  \label{eq:two}
    \end{align}

    Since $\Ualter$ is within the safety margin of $\U$, their Shapley value ranking is the same. 
    Hence, $\phiS$ is also the set of data points that achieve the highest Shapley value under $\Ualter$. 
    Moreover, due to the form of $\Ualter$, we know that 
    \begin{align}
        \phiS &= \argmax_{S: |S|=k} \Ualter(S) \label{eq:three}
    \end{align}
    Hence we have $\Ualter(\phiS) \ge \Ualter(\optS^{(k)})$. Combining with (\ref{eq:one}) and (\ref{eq:two}) gives us 
    \begin{align*}
        \U( \phiS ) \ge \U( \optS^{(k)} ) - 2 \norm{\Ualter - \U}
    \end{align*}
\end{proof}


==> noise_stab_theorem_for_fixed_f.tex <==
\begin{theorem}
\label{thm:fit-residual-bound-main}
Denote the monotonic function class $\F_\gamma = \{ f: 
\frac{\max_t f'(t)}{\min_t f'(t)} = \gamma, \min_t f'(t)>0\}$. 
Denote the subclass of monotonically transformed modular function defined on $\dataset$ as $\M_\gamma = \{\U: \U(S) = f(w_0 + \sum_{i \in S} w_i), f \in \F\}$. 
Let $\gamma := U/L$. Then we have 
\begin{align*}
    \min_{\Ualter \in \M_\gamma} \normR(\Ualter) 
    \le 
    \frac{1}{1-\rho^2} \left( \gamma^2 + \disc(\U) \right)
\end{align*}
for any $\rho \in (0, 1)$, where 
\begin{equation}
\resizebox{\columnwidth}{!}{
$\begin{aligned}
    \disc(\U) := \frac{ \gamma^2 \E_{S \sim \unif(\dataset)} \left[ \U(S) \right]^2 - \underset{\substack{S \sim \unif(\dataset) \\ S' \sim \sampleRho(S)}}{\E} \left[ \U(S) \U(S') \right] }{ \Var_{S \sim \unif(\dataset)}(\U(S)) }
\end{aligned}$
} \nonumber
\end{equation}
% \begin{align*}
%     \disc(\U) := \frac{ \gamma^2 \E_{S \sim \unif(\dataset)} \left[ \U(S)^2 \right] - \underset{\substack{S \sim \unif(\dataset) \\ S' \sim \sampleRho(S)}}{\E} \left[ \U(S) \U(S') \right] }{ \Var_{S \sim \unif(\dataset)}(\U(S)) }
% \end{align*}
is the \emph{normalized norm-stability discrepancy} for $\U$. 
% \begin{align*}
%     & \min_{\Ualter \in \M} 
%     \frac{ \E_{S \sim \unif(\dataset)} \left[ \left(\U(S) - \Ualter(S)\right)^2 \right] }{ \Var_{S \sim \unif(\dataset)}(\U(S)) } \\
%     &\le 
%     \frac{1}{1-\rho^2} \left( \gamma^2 + \frac{ \gamma^2 \E_{S \sim \unif(\dataset)} \left[ \U(S)^2 \right] - \underset{\substack{S \sim \unif(\dataset) \\ S' \sim \sampleRho(S)}}{\E} \left[ \U(S) \U(S') \right] }{ \Var_{S \sim \unif(\dataset)}(\U(S)) } \right)
% \end{align*}
% for any $\rho \in (0, 1)$. 
\end{theorem}
